Runtime Stealthy Perception Attacks against DNN-based Adaptive Cruise Control Systems

Adaptive Cruise Control (ACC) is a widely used driver assistance technology for maintaining the desired speed and safe distance to the leading vehicle. This paper evaluates the security of the deep neural network (DNN) based ACC systems under runtime stealthy perception attacks that strategically inject perturbations into camera data to cause forward collisions. We present a context-aware strategy for the selection of the most critical times for triggering the attacks and a novel optimization-based method for the adaptive generation of image perturbations at runtime. We evaluate the effectiveness of the proposed attack using an actual vehicle, a publicly available driving dataset, and a realistic simulation platform with the control software from a production ACC system, a physical-world driving simulator, and interventions by the human driver and safety features such as Advanced Emergency Braking System (AEBS). Experimental results show that the proposed attack achieves 142.9 times higher success rate in causing hazards and 82.6% higher evasion rate than baselines, while being stealthy and robust to real-world factors and dynamic changes in the environment. This study highlights the role of human drivers and basic safety mechanisms in preventing attacks.

==> comparison-table.tex <==
\begin{table}[h!]
\footnotesize
\centering

\caption{Comparison of Attack Approaches Targeting DNN Perception or ADAS.}
%\homa{Separated into two columns and differentiated  runtime attacks. }} 
\label{tab:comparison}
\resizebox{\columnwidth}{!}
{%
\small
\begin{threeparttable}
    
\begin{tabular}{lllllll}
\toprule
\textbf{Attack} &   \multicolumn{3}{c}{\textbf{Attack} }& \multicolumn{2}{c}{\textbf{Safety Interventions}} & \textbf{Autonomy} \\  \cmidrule(lr){2-4}  \cmidrule(lr){5-6}
 \textbf{Method}& \textbf{Type}& \textbf{Vector}&\textbf{Target}& \textbf{AEBS} & \textbf{Driver} &\textbf{Level}\cite{SAEroadmap}\\
\midrule
\citet{eykholt2018robust}  & \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Offline\end{tabular}}& Stickers on road signs  &Classifier & N & N &N/A\\
\citet{ma_wip_2023}        && Patch projected         &MTO& N & N & L4\\
\citet{tencent2019experimental} && Stickers on road  &ALC & N & N &L2\\
\citet{guo2023adversarial} && Patch on truck  &ACC & N & N & L2\\ %, Apollo (no ACC)
 \citet{sato2021dirty} & & Patch on road  & ALC & \textbf{Y} & N &L2\\ \midrule

\citet{jia2019fooling} & \multirow{4}{*}{Run-time}& Perception inputs  &MTO & N & N & L4\\
\citet{jha2020ml}  & & Perception inputs  &MTO & No FCW & N &L4\\
\citet{ma2021sequential} & & Inner state variables &FCW & No AEB & Y &N/A\\
\citet{zhou2022strategic}  & & Control commands  &ACC, ALC & No AEB& \textbf{Y} &L2\\
Our work  & & Perception inputs  &ACC & \textbf{Y} & \textbf{Y} &L2\\
\bottomrule
\end{tabular}%

\begin{tablenotes}
    \item[*]MTO: Multi-Object Tracking;% KF: Kalman Filter.
\end{tablenotes}

\end{threeparttable}

}
\end{table}

